Bs and Bc mesons in lattice QCD with exact chiral symmetry

We determine the masses and decay constants of the pseudoscalar mesons Bs and Bc, and also the masses of the vector mesons Bs^* and Bc^*, in quenched lattice QCD with exact chiral symmetry. For 100 gauge configurations generated with single-plaquette action at beta = 7.2 on the 32^3 x 60 lattice, we compute point-to-point quark propagators for 33 quark masses in the range [0.01, 0.85], and measure the time-correlation functions of pseudoscalar and vector mesons. The inverse lattice spacing and the charm quark bare mass are determined using the mass and decay constant of eta_c(2980). The bare masses of s and b quarks are chosen such that the masses of the corresponding vector mesons are in good agreement with phi(1020), and Upsilon(9460) respectively. Our results are: m_{Bs} = 5385(27)(17) MeV, f_{Bs} = 253(8)(7) MeV, m_{Bc} = 6278(6)(4) MeV, f_{Bc} = 489(4)(3) MeV, m_{Bs^*} = 5424(28)(19) MeV, and m_{Bc^*} = 6315(6)(5) MeV.

==> PoS.cls.2005 <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% PoS.cls 1.1.1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This file is Copyright PoS 2005:  it can be freely distributed  but
%% NOT modified preserving its name, even in similar forms.
%% 
%% PoS.cls is a LaTeX2e class file used to typeset manuscripts in PoS - 
%% Proceedings of Science style. It was written by P. Dall'Aglio as a 
%% modification of the class `JHEP3.cls'.
%% 
%% For bugs, comments, suggestions email to pos-eo@pos.sissa.it
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ***:to do  **?:question  ...:to choose  XXX:to delete  ???:unknown %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01] \ProvidesClass{PoS} [2005/05/09
v1.1.1 LaTeX document class - P.D.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\logo{\raisebox{-5mm}{\hbox{\noindent\includegraphics{PoSlogo}}}}
%\def\logo{\raisebox{-5mm}{\hbox{\noindent\special{psfile=PoSlogo.ps}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW SWITCHES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@draft   \@draftfalse			% DEFAULT IS NOT DRAFT
\newif\if@hyper   \@hypertrue			% DEFAULT IS HYPER
\newif\if@proc	  \@proctrue			% DEFAULT IS PROC

\newif\if@author\@authorfalse			%
\newif\if@abstract\@abstractfalse		% FOR FRONTMATTER DECLARATIONS
\newif\if@todotoc\@todotocfalse			%
\newif\if@PoScopy\@PoScopyfalse			%
\newif\if@PoS\@PoSfalse			%
\newif\if@conf\@conffalse			%
\newif\if@shorttitle\@shorttitlefalse			%
\newif\if@PoSspecialurl\@PoSspecialurlfalse
\newif\if@PoScits\@PoScitsfalse			%
\@twocolumnfalse

\if@compatibility
    \setlength\paperheight {297mm}%		% DEFAULT FOR LATEX209 IS a4
    \setlength\paperwidth  {210mm}%
\else						% CHOSE PAPER:
\DeclareOption{a4paper}
   {\setlength\paperheight {297mm}%
    \setlength\paperwidth  {210mm}}
\DeclareOption{a5paper}{\@OImess{}}		% IGNORED a5
\DeclareOption{b5paper}{\@OImess{}}		% IGNORED b5
\DeclareOption{letterpaper}
   {\setlength\paperheight {11in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{legalpaper}
   {\setlength\paperheight {14in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{executivepaper}
   {\setlength\paperheight {10.5in}%
    \setlength\paperwidth  {7.25in}}
\DeclareOption{landscape}{\@OImess{}}		% IGNORED landscape
\fi

\newcommand\@ptsize{1}                          % DEFAULT SIZE IS 11 PT

\DeclareOption{proceedings}{\@hypertrue\AtBeginDocument{\@todotocfalse}}

\DeclareOption{hyper}{\@hypertrue\@OImess{ is automatic in PoS}}	% HYPER IS 11 PT
\DeclareOption{nohyper}{\@hyperfalse\PoS@warnl{Option `hyper' should be used}}	% IGNORED nohyper
\DeclareOption{11pt}{\renewcommand\@ptsize{1}\@NFmess{11pt}} %ALWAYS 11PT
\DeclareOption{12pt}{\renewcommand\@ptsize{1}\@NFmess{11pt}}% ALWAYS 11PT
\DeclareOption{10pt}{\renewcommand\@ptsize{1}\@NFmess{11pt}}% ALWAYS 11PT

\DeclareOption{nocits}{\@OImess{ is default for PoS}
                     \@PoScitsfalse}

\DeclareOption{cits}{\@PoScitstrue}

%%%% ??????????????
%come fare per disabilitare cite e forzare cits?
%%%%????????????????????

\if@compatibility\else
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}\fi
\DeclareOption{twoside}{\@OImess{}}
\DeclareOption{notoc}{\AtBeginDocument{\@todotocfalse}
			\@OImess{ is automatic in PoS}}
\DeclareOption{toc}{\AtBeginDocument{\@todotoctrue}}

\DeclareOption{draft}{\setlength\overfullrule{5pt}% EXTENDED DRAFT
	\newcount\hour\newcount\minute
	\hour=\time \divide\hour by60 \minute=\time
	{\multiply\hour by60 \global\advance\minute by-\hour}
	\edef\militarytime{\number\hour:\ifnum\minute<10 0\fi\number\minute}
	\let\old@eqnnum\@eqnnum
	\def\@eqnnum{\old@eqnnum\rlap{\kern\marginparsep
				\if@twocolumn\if@firstcolumn
				  \kern-2\marginparsep\kern-\columnwidth\
				  \llap\bgroup\else\bgroup\fi
				\else
				\if@twoside\ifodd\c@page
				  \kern-2\marginparsep\kern-\textwidth
				  \llap\bgroup\else\bgroup\fi
				\else\bgroup\fi				
				\fi
				\sf\scriptsize\@eqnlabel\egroup}%
				\gdef\@eqnlabel{}}
	\let\@eqnlabel\relax
	\def\math@note#1{\gdef\@eqnlabel{LAB: #1}}
	\def\norm@note#1#2{\special{}% SORRY AGAIN.
			 \ifinner{\ifdim\baselineskip=\z@% IN ARRAY..
					\baselineskip18\p@\fi%%
				\ifhmode%   ATTENTION TO RESTRICTED VMODE!
				\raisebox{.5\baselineskip}[\z@][\z@]{%
					\rlap{\sf\scriptsize #2}}%
				\else\vskip-\baselineskip%
				\raisebox{-.6\baselineskip}[\z@][\z@]{%
						\rlap{\sf\scriptsize #2}}%
				\fi}%
			 \else\marginpar{\raggedright\if@twoside\ifodd\c@page%
					\raggedleft\fi\fi\sf\scriptsize #1#2}%
			 \fi}%
	\AtBeginDocument{\newbox\drft@box\setbox\drft@box=\hbox{%
			\framebox[\textwidth]{\sf\small PoS 3.1 DRAFT 
			\ttfamily(\cur@opt)\hfill\sf\bfseries\jobname\sf, 
			\today, \militarytime}}}
	\@drafttrue}

\DeclareOption{titlepage}{\@OImess{}}		% IGNORED
\if@compatibility\else
\DeclareOption{notitlepage}{\@OImess{}}		% IGNORED
\fi
\if@compatibility\else
\DeclareOption{onecolumn}{\@OImess{}}		% IGNORED
\fi
\DeclareOption{twocolumn}{\@OImess{}}		% IGNORED
\DeclareOption{leqno}{\@OImess{}}	%\input{leqno.clo}} IGNORED ...
\DeclareOption{fleqn}{\@OImess{}}	%\input{fleqn.clo}} IGNORED ...
\DeclareOption{openbib}{\@OImess{}}		% IGNORED


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MESSAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\PoS@mess[1]{\typeout{Class PoS Message: \protect#1.}}%
\newcommand\PoS@warn[1]{\ClassWarning{PoS}{#1}}
\newcommand\PoS@warnl[1]{\ClassWarningNoLine{PoS}{#1}}
\newcommand\PoS@igno[1]{\PoS@warn{IGNORED \protect#1}}
\newcommand\PoS@ignol[1]{\PoS@warnl{IGNORED \protect#1}}
\newcommand\@OImess[1]{\PoS@ignol{OPTION '\CurrentOption'#1}}
\newcommand\@NFmess[1]{\PoS@mess{Normalsize set to #1}}
\newcommand\@ENVwarn[1]{\PoS@warn{Please use \protect#1 in place 
						of LaTeX environment}}
%%%%%%%%%%%%%%%%%%%%%%%%%% PROCESS OPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ExecuteOptions{a4paper,oneside,proceedings} %WERE ALSO 10pt,onecolumn
\ProcessOptions

%%%%%%%%%%%%%%%%%%%%%%%%%% REQUIRED PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{amssymb}
\RequirePackage[T1]{fontenc}
\RequirePackage{times}
\RequirePackage{mathptmx}
\RequirePackage{color}
\RequirePackage{ifpdf}
\ifpdf
      \RequirePackage[pdftex]{graphicx}
      \DeclareGraphicsExtensions{.pdf,.jpg,.jpeg}
\else
      \RequirePackage{graphicx}
      \DeclareGraphicsExtensions{.ps,.eps,.pstex}
\fi
%%%%%%%%%%%%%%%%%%%%%%%% TRICKS FOR DOTLESS J %%%%%%%%%%%%%%%%%%%%%%%%%
% \j and \jmath are missing in font Times. So I use the ones from
% Computer Modern. Works acceptably, but in sf
\DeclareSymbolFont{forjmath}{OT1}{cmr}{m}{sl}
\DeclareMathSymbol{\Jmath}{\mathord}{forjmath}{'021}
\def\jmath{\Jmath}
\DeclareFontFamily{OT1}{cmr}{}
\DeclareFontFamily{OT1}{cmss}{}
\def\j{\ifmmode\Jmath\else{\fontencoding{OT1}\fontfamily{cmr}\selectfont\char'021}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% END DOTLESS J %%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% START CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{size1\@ptsize.clo}
\renewcommand{\baselinestretch}{1.1}\normalsize
\setlength\lineskip{1\p@}
\setlength\parindent{1.2\parindent}
\setlength\normallineskip{1\p@}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\widowpenalty 1000
\clubpenalty 1000

\setcounter{topnumber}{8}
\renewcommand\topfraction{.85} % default .7
\setcounter{bottomnumber}{5}
\renewcommand\bottomfraction{.6} %.2
\setcounter{totalnumber}{8}
\renewcommand\textfraction{.15}
\renewcommand\floatpagefraction{.8}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.85}
\renewcommand\dblfloatpagefraction{.8}
\setlength{\floatsep}{12pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{20pt plus 3pt minus 8pt}
\setlength{\intextsep}{12pt plus 2pt minus 4pt}

\textwidth  .72\paperwidth	% WIDTH OF TEXT, REMAINS .28% FOR MARGINS
%
\setlength\@tempdima{.76\paperheight}	% HEIGHT OF TEXT WITH FOOTNOTES
\divide\@tempdima\baselineskip		% EXCLUDING HEAD (AND FOOT)
\@tempcnta=\@tempdima			% rounded to integer (#lines-1)
\setlength\textheight{\@tempcnta\baselineskip}
\addtolength\textheight{\topskip}

\voffset -1in
\topmargin   .06\paperheight	% FROM TOP OF PAGE TO TOP OF HEADING (0=1inch)
\headheight  .02\paperheight	% HEIGHT OF HEADING BOX.
\headsep     .03\paperheight	% VERT. SPACE BETWEEN HEAD AND TEXT.
\footskip    .04\paperheight	% FROM END OF TEX TO BASE OF FOOTER. (40pt)

\marginparsep 9\p@		% HOR. SPACE BETWEEN TEXT AND MARGINAL NOTE
\marginparpush 6\p@		% MIN. VERT. SPACE BETWEEN MARGINAL NOTES

\hoffset -1in				% TO ADJUST WITH PAPER:

	\oddsidemargin .14\paperwidth	% LEFT MARGIN FOR ODD PAGES (20)
	\evensidemargin .14\paperwidth	% LEFT MARGIN FOR EVEN PAGES (20)
	\marginparwidth .11\paperwidth	% TEXTWIDTH OF MARGINALNOTES

%%%%%%%%%%%%%%%%%%%%%%% HYPER (AND DRAFT) STUFF %%%%%%%%%%%%%%%%%%%%%%%
%\let\textref\@gobble
\ifpdf
      \input pdfcolor.tex
\else
\fi

\bgroup\catcode`\#=12\gdef\hash{#}\egroup	% DEFINED \hash=#.
\def\H@tilde{\string~}
\newcommand{\href}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
		      \if@hyper\ifpdf
				    \def\hash{}%
				    \pdfstartlink attr{/Border [0 0 0]}
                                    user{/Subtype /Link /A << /S /URI /URI (#1) >>}%
					\pdfsetcolor{.9 .9 0 0}%
				\else
				    \noexpand\special{html:<A href="#1">}%
				\fi
		      \fi
		      {#2}\rule{0pt}{0pt}\egroup
		      \if@hyper\ifpdf
				    \Black\pdfendlink
			       \else
				    \special{html:</A>}%
			       \fi
                      \fi
		      }
% \intPlink was added because in pdflatex you need two different commands
% for internal and external llinks. For latex they are the same.
\newcommand{\intPlink}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
                        \if@hyper\ifpdf
                                       \def\hash{}%
                                       \pdfstartlink attr{/Border [0 0 0]}
                                          goto name{#1}%
                                       \pdfsetcolor{.9 .9 0 0}%
				  \else
                                       \noexpand\special{html:<A href="#1">}%
				  \fi
			\fi
                        {#2}\rule{0pt}{0pt}\egroup
                        \if@hyper\ifpdf
                                      \Black\pdfendlink
				 \else
                                      \special{html:</A>}%
                                 \fi
                        \fi
                        }


\newcommand{\name}[1]{\if@hyper\ifpdf
				    \pdfdest name{#1} fith%
			       \else
				    \noexpand\special% NAME HAS NO TAGGED TEXT HERE.
					{html:<A name="#1">}\special{html:</A>}%
			       \fi
		      \fi
		      }

\newcommand{\base}[1]{\if@hyper\bgroup\let~\H@tilde
			\noexpand\special	% BASE HAS NO TAGGED TEXT.
			{html:<base href="#1">}\egroup\fi}
%------------------------------------------------------------------%
% SECTION TAGS and  THEIR REFERENCE IN TOC \d@t will be '.' for sections only
\if@hyper
\renewcommand{\@seccntformat}[1]{\name{sec\csname the#1\endcsname}%
				 \csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{\intPlink
			      {\hash\hyp@typ#1}{#1}\d@t\hfil}}
\else
\renewcommand{\@seccntformat}[1]{\csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{#1\d@t\hfil}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% per avere le citazioni che collassano %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% scommentare da qui %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\if@PoScits
\newcount\@tempcntc
\def\@citex[#1]#2{%
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}%
  \@cite{\@for\@citeb:=#2\do%                                               for aech citation...
         {\edef\@citeb{\expandafter\@firstofone\@citeb}%                    eat trailing space
          \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi% write to aux
          \@ifundefined{b@\@citeb}%                                         if label undefined..
                       {\@citeo\@tempcntb\m@ne\@citea%                      ... then ...
                        \def\@citea{,\penalty\@m\ }{\reset@font\bfseries ?}%
	                \G@refundefinedtrue\@latex@warning%
                        {Citation `\@citeb' on page \thepage \space undefined}}%
                       {\setbox\z@\hbox{\global\@tempcntc0\csname %         ... else
                                        b@\@citeb\endcsname}%
                        \advance\@tempcntb\@ne%
                        \ifnum\@tempcntb=\@tempcntc%
                        \else\advance\@tempcntb\m@ne\@citeo%
                             \@tempcnta\@tempcntc\@tempcntb\@tempcntc
                        \fi%
                        }%
         }\@citeo}{#1}%
	 \if@draft\norm@note{CIT: }{#2}\fi			% **DRAFT**
    }% end definition of \@citex
%This really prints out the cit-numbers
\def\@citeo{\ifnum\@tempcnta>\@tempcntb%    
            \else\@citea\def\@citea{,\penalty\@m\ }%
                  \ifnum\@tempcnta=\@tempcntb%
                  \intPlink{\hash bib\the\@tempcnta}{\the\@tempcnta}% if there is no range
                  \else{\advance\@tempcnta\@ne%                 % if there is a range
                       \ifnum\@tempcnta=\@tempcntb%
                       \else\def\@citea{\,--\,}%
                       \fi%
                       \advance\@tempcnta\m@ne%
                       \intPlink{\hash bib\the\@tempcnta}{\the\@tempcnta}\@citea%first
                       \intPlink{\hash bib\the\@tempcntb}{\the\@tempcntb}}%last
                  \fi%
             \fi}
%%%%%%%%%%%%%%% fino a qui %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------------------------------------------------%
% CITATION TAGS ARE TOGETHER WITH BIB STUFF.
% CITATION HREF
\else %perche' sta qui e non 6 righe piu` sopra? ???????
\def\@citex[#1]#2{%			% UNFORTUNATELY REDEFINED!!!!
  \let\@citea\@empty
  \@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{,\penalty\@m\ }%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb}{\mbox{\reset@font\bfseries ?}%
	\G@refundefinedtrue
	\@latex@warning
	  {Citation `\@citeb' on page \thepage \space undefined}}%
	{\edef\tmp@bn{\csname b@\@citeb\endcsname}%
	 \hbox{\intPlink{\hash bib\tmp@bn}{\tmp@bn}}}}}{#1}%		% **HYPER**
	 \if@draft\norm@note{CIT: }{#2}\fi			% **DRAFT**
	 }
\fi

%-----------------------------------------------------------------%
% LABEL, REF AND PAGEREF, TEXTREF, ~ COMPATIBLE:
\let\old@label\label						% OLD LATEX COMMAND.
\def\label{\bgroup\catcode`\>=15\catcode`\"=15\catcode`\==15 \@@label}		
\newcommand{\@@label}[1]{\egroup\name{ref-#1}%		% LABEL IN HYPER TAG.
			 \old@label{#1}%		% 
			 \if@draft%			% DRAFT:
			 \ifmmode\math@note{#1}%
			 \else\norm@note{}{LAB: #1}\fi%
			 \fi%
			 }
\if@hyper
\let\old@ref\ref \let\old@pageref\pageref		% OLD LATEX COMMANDS.
\renewcommand{\ref}[1]{\@ifundefined{r@#1}{}{\intPlink{\hash ref-#1}}%
		       {\old@ref{#1}}} % LABEL INSIDE HREF.
\renewcommand{\pageref}[1]{\@ifundefined{r@#1}{}{%	% UNDEFINED => NO HREF
	      \edef\tmp@ref{\noexpand\@secondoftwo\csname r@#1\endcsname}%
	      \intPlink{\hash pag\tmp@ref}}{\old@pageref{#1}}}
\fi
\newcommand{\textref}[2]{\@ifundefined{r@#1}
			{%
			\protect\G@refundefinedtrue
			\nfss@text{\reset@font\bfseries ?#2?}%
   			\@latex@warning{Reference `#1' on page \thepage \space
				             undefined}}
			{\vrule height \z@ width \z@\intPlink{\hash ref-#1}{#2}}}
%------------------------------------------------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%% END HYPER-STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% PoS HEADINGS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ps@PoS{% 			
    \def\@oddfoot{\ifnum\thepage=1%
		{\bop}\PoScopyright@box\hfill% copyright only on front page of published papers
		\if@PoSspecialurl\PoSspecial@url\else\unhbox\PoSpaper@url\fi%possible url
		\else\bop\reset@font\hfil \copy\PoSacce@number\ /\ \thepage\hfil\fi} % page numbers on other pages
    \if@draft\edef\cur@opt{\@curroptions}\fi
%
    \def\@oddhead{\name{pag\thepage}\ifnum\thepage=1%
      {\smash{\makebox[0cm][l]{\logo}}\hfill}\else%
      \smash{\if@draft\raise 2.5em\rlap{\copy\drft@box}\fi
		     \vbox{\hsize=\textwidth\noindent
		     \if@shorttitle\copy\PoSshorttitle@box\else{\small\it\@title}\fi\hfill
		     \copy\@firstaubox\vskip.17em \hrule
             }}\fi%
		      }%
    \let\@mkboth\@gobbletwo  %%%% 
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TITLE PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maketitle{\PoS@ignol{\maketitle}}
\newcommand\auto@maketitle{\begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}% 
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}% 
    \long\def\@makefntext##1{\parindent 20.39995pt\noindent
            \hb@xt@.05\textwidth{\hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
    \let\footnote\thanks%
	 \@maketitle				% CALL ACTUAL FORMATTING
	 \@thanks				% TITLE THANKS
	 \thispagestyle{PoS} 
 	 \setcounter{page}{1}
	 \newpage				% END OF PAGE
  \endgroup
  \setcounter{footnote}{0}%			
  \if@todotoc					% IF THERE IS A SECTION
      \noindent\rule\textwidth{.1pt}		% THEN MAKE TOC...
      \vskip 2em \@plus 3ex \@minus 3ex
      \tableofcontents
      \vskip 2em \@plus 3ex \@minus 3ex
      \noindent\rule\textwidth{.1pt}
      \vskip 2em \@plus 3ex \@minus 3ex
  \fi
  \global\let\thanks\@gobble
  \global\let\@maketitle\relax			%
  \global\let\@thanks\@empty			%
  \global\let\@author\@empty			% KILL ALL 
  \global\let\@date\@empty			%
  \global\let\@abstract\@empty			%
  \global\let\title\relax			%
  \global\let\author\relax			%
  \global\let\date\relax			%
  \global\let\and\relax				%
  \global\let\email\@gobble
  \global\let\PoScopydate\relax
  \global\let\PoSspecialurl\relax
}
%%%%%%%%%%%%%%%%%%%%%%%%%% ACTUAL TITLEPAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newskip\titlesk@a		% Skips for titlepage
\newskip\titlesk@b		%
\newskip\titlesk@c		%
\titlesk@a= 2em   plus .4fill  minus 1em%	% Before title (proceedings)
\titlesk@b= 1.7em plus .1fill  minus 1em%	% Between title/rule & rule/auth
\titlesk@c= 1.5em plus .05fill minus 1em%	% Between auth/abs & abs/dedic

\def\@maketitle{%				% PAGE IS FLUSHED LEFT
  \begin{flushleft}%				% PAY ATTENTION TO \par'S
    \null
    %
    \vskip \titlesk@a		   % vspace before title
    %
    {\LARGE \sffamily              % TITLE  
      \bfseries                  
      \@title\par}%                
    %
    \vskip \titlesk@b              % vspace between title and rule
    %
    \hrule height 1\p@%            % RULE  1pt.
    %
    \vskip \titlesk@b		   % vspace between rule and authors
    %
    {\normalsize \bfseries \sffamily% AUTHOR(S)
      \@author \par}                            
    %
    \vskip \titlesk@c              % vspace between authors and abstract
    %
    \centerline{\parbox{.9\textwidth}%	% ABSTARCT (narrower)
      {\abstract@cs}}%
    %
    \dedic@ted                     % DEDICATION (if present) with its space
    %
    \@PACS                         % PACS (if present) with its space
    %
    \vskip \titlesk@c            
    \vfill
    \FullConference@box            % FULL CONFERENCE INFO
  \end{flushleft}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%% STANDARD STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{secnumdepth}{3}
\newcounter {part}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thepart         {\@Roman\c@part}
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION FORMATS %%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ts@flag{\let\d@t.%					% Sections get ``.''
	     \immediate\write\@auxout			% IF THERE IS A SECTION
	     {\string\global\string\@todotoctrue}}	% THEN SIGNAL IN AUX.

\newcommand\part{\par
   \addvspace{4ex}%
   \@afterindentfalse
   \secdef\@part\@spart}

\def\@part[#1]#2{\ts@flag
    \ifnum \c@secnumdepth >\m@ne
      \refstepcounter{part}%			% DAMN LATEX !!! BELOW,
      \addcontentsline{toc}{part}{\string\intPlink	% UNFORTUNATELY, NO NUMBERLINE:
				  {\string\hash\space part\the\c@part}%
				  {\thepart}\hspace{1em}#1}%
    \else
      \addcontentsline{toc}{part}{#1}%
    \fi
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \ifnum \c@secnumdepth >\m@ne
       \name{part\the\c@part}\Large\bfseries \partname~\thepart
       \par\nobreak
     \fi
     \huge \bfseries #2%
     \markboth{}{}\par}%
    \nobreak
    \vskip 3ex
    \@afterheading\let\d@t\relax}
\def\@spart#1{%
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \huge \bfseries #1\par}%
     \nobreak
     \vskip 3ex
     \@afterheading}

\newcommand\secstyle{\bfseries\raggedright}

\newcommand\section{\@startsection{section}{1}{\z@}%
                                   {3.5ex \@plus 1.3ex \@minus .7ex}%
                                   {2.3ex \@plus.4ex \@minus .4ex}%
                                   {\normalfont\large\secstyle}}
\newcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {2.3ex\@plus 1ex \@minus .5ex}%
                                   {1.2ex \@plus .3ex \@minus .3ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {2.3ex\@plus 1ex \@minus .5ex}%
                                   {1ex \@plus .2ex \@minus .2ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {1.75ex \@plus1ex \@minus.2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}
\newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
                                   {1.75ex \@plus1ex \@minus .2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}

% ---- turnaround for sections with figures ------ %
\def\bef@sec{\iffigprocessing\PoS@warnl{Floating figure \the\ffigcount\space
						and startsection colliding}\fi
	     \iftabprocessing\PoS@warnl{Floating table \the\ftabcount\space
						and startsection colliding}\fi
	     \edef\bef@everypar{\the\everypar}}	% HACK FOR FLOATS AND \everypar
\def\aft@sec{\let\d@t\relax			% RESTORE: NO DOTTED SUBSECS..
	     \edef\tmp@everypar{\the\everypar}% % DELETED CLUBPENALTY, BELOW.
	     \everypar\expandafter{\bef@everypar{\tmp@everypar}}}% RESTORE.
\let\old@sec\section				%
\let\old@ssec\subsection			%
\let\old@sssec\subsubsection			% OLD SECTIONING COMMANDS.
\let\old@par\paragraph				%
\let\old@spar\subparagraph			%
% ------- new forms ------- %
\renewcommand{\section}{\secdef\PoS@sec\PoS@secs}
\renewcommand{\subsection}{\secdef\PoS@ssec\PoS@ssecs}
\renewcommand{\subsubsection}{\secdef\PoS@sssec\PoS@sssecs}
\renewcommand{\paragraph}{\secdef\PoS@par\PoS@pars}
\renewcommand{\subparagraph}{\secdef\PoS@spar\PoS@spars}
% ---- unstarred forms ---- %
\def\PoS@sec[#1]#2{\ts@flag\bef@sec\old@sec[#1]{#2}\aft@sec}
\def\PoS@ssec[#1]#2{\bef@sec\old@ssec[#1]{#2}\aft@sec}
\def\PoS@sssec[#1]#2{\bef@sec\old@sssec[#1]{#2}\aft@sec}
\def\PoS@par[#1]#2{\bef@sec\old@par[#1]{#2}\aft@sec}
\def\PoS@spar[#1]#2{\bef@sec\old@spar[#1]{#2}\aft@sec}
% ----- starred forms ----- %
\def\PoS@secs#1{\bef@sec\old@sec*{#1}\aft@sec}
\def\PoS@ssecs#1{\bef@sec\old@ssec*{#1}\aft@sec}
\def\PoS@sssecs#1{\bef@sec\old@sssec*{#1}\aft@sec}
\def\PoS@pars#1{\bef@sec\old@par*{#1}\aft@sec}
\def\PoS@spars#1{\bef@sec\old@spar*{#1}\aft@sec}
% ----- end hack for sections with floats --------%

\setlength\leftmargini  {2.5em}
\leftmargin  \leftmargini
\setlength\leftmarginii  {2.2em}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
  \setlength\leftmarginv  {1em}
  \setlength\leftmarginvi {1em}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}
\newcommand\labelitemi{$\m@th\bullet$}
\newcommand\labelitemii{\normalfont\bfseries --}
\newcommand\labelitemiii{$\m@th\ast$}
\newcommand\labelitemiv{$\m@th\cdot$}
\newenvironment{description}
               {\list{}{\labelwidth\z@ \itemindent-\leftmargin
                        \let\makelabel\descriptionlabel}}
               {\endlist}
\newcommand*\descriptionlabel[1]{\hspace\labelsep
                                \normalfont\bfseries #1}
%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHORS/ADDRESSES %%%%%%%%%%%%%%%%%%%%%%%%%%
% *** After proceedings, the authors go in a hbox. => \break does not work!!
% *** if no address nobody closes the box!
\newif\if@speaker\@speakerfalse
\newif\if@dblspeak\@dblspeakfalse
\newtoks\prev@t
\newtoks\cur@t
\newbox\@firstaubox
\newskip\addr@skip\addr@skip=.38em%\@plus.02fil\@minus.3ex
\newskip\auth@skip\auth@skip=.6em\@plus.03fil\@minus.2ex

\renewcommand\@author{\parskip\z@
		      \def\\{\egroup			% CLOSE & aftergroup!
			\par				% FIRST TIME \\=>ADDR.
			\vskip\addr@skip		% GLUE UNDER AUTHOR
			\vbox\bgroup\hsize=.9\textwidth	% 
			\small\it\raggedright		% STYLE FOR ADDRESSES
			\def\\{\par\leavevmode\ignorespaces}%\let\\\relax%
			\leavevmode\ignorespaces}%
			}
\renewcommand\author[1]{%
		\global\@authortrue			%
		\prev@t=\expandafter{\@author}%		% TWO TOKEN LISTS.
		\cur@t={\vskip\auth@skip		% glue before auth.
			\vtop\bgroup #1\egroup		% ACTUAL AUTH.\\ADD.
			\par}%				%
		\long\xdef\@author{\the\prev@t\the\cur@t}%STORE ALL IN \@AUTHOR
		}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPEAKER %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\speaker[1]{\if@speaker\global\@dblspeaktrue\fi
			\global\@speakertrue
			\global\setbox\@firstaubox
			\hbox{{\let\thanks\@gobble
				\let\footnote\@gobble\small 
				\rm #1}}%
			#1\thanks{Speaker.}\
			}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SHORT TITLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\PoSshorttitle@box
\newcommand\ShortTitle[1]{\global\setbox\PoSshorttitle@box
                          \hbox{\small\it #1}\global\@shorttitletrue}
%%%%%%%%%%%%%%%%%%%%%%%%%% Full Conference Info %%%%%%%%%%%%%%%%%%%%%%%
\gdef\FullConference@box{\relax}
\newcommand\FullConference[1]{\gdef\FullConference@box{
			 \vbox{\small\raggedright
			   \it #1}}\@conftrue}
%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT DATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\PoScopy@date
\newcommand\PoScopydate[1]{\global\setbox\PoScopy@date
                        \hbox{\scriptsize #1}\global\@PoScopytrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%% ACKNOWELEDGMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\acknowledgments{\section*{\acknowlname}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EMAIL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\email[1]{{\tt\href{mailto:#1}{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEDICATED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\dedic@ted{\relax}
\newcommand\dedicated[1]{\gdef\dedic@ted{\vskip .5\titlesk@c
                              \vbox{\small\it\raggedleft #1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PACS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\@PACS{\relax}
\newcommand\PACS[1]{\gdef\@PACS{\vskip.5\titlesk@c
                                \vbox{\small\tt\raggedleft PACS:\ #1}}} 
%%%%%%%%%%%%%%%%% SPECIAL URL overrides paper@url %%%%%%%%%%%%%%%%%%%%%
\gdef\PoSspecial@url{\relax}
\newcommand\PoSspecialurl[1]{\@PoSspecialurltrue\gdef\PoSspecial@url{%
    \hbox{\tiny\tt #1}}}
%%%%%%%%%%%%%%%%%%%%%%%%% FILE NAME AND URL %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\PoSconf@acro
\newbox\PoSacce@number
\def\PoSsplit@ident PoS(#1)#2.{\setbox\PoSconf@acro\hbox{\rm #1} % not used
			 \setbox\PoSacce@number\hbox{\rm #2}} % used in page number

\newbox\PoSpaper@url

\global\setbox\PoSpaper@url\hbox{\tiny\ttfamily 
		http://pos.sissa.it/}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\PoScopyright@box{\hbox{{\tiny $\copyright$ Copyright owned by
the author(s) under the terms of the Creative Commons
Attribution-NonCommercial-ShareAlike Licence.}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABSTRACT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\abstract}[1]%		% ABSTR. IN NORMALSIZE
	{\gdef\abstract@cs{		% cs FOR WHOLE ABSTRACT
	{\small
	  \ignorespaces #1}}
	\normalsize
	\global\@abstracttrue}
%%%%%%%%%%%%%%%%%%%%%%%%%% OTHER ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{verse}
               {\let\\\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item\relax}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item\relax}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@xthm#1#2{\@begintheorem{#2}		 % theorems are numbered
		{\csname the#1\endcsname.}	 % with a . after the number
		\ignorespaces}

\newcommand\Proof{\noindent\emph{Proof.}\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% SOME MORE LENGHTS %%%%%%%%%%%%%%%%%%%%%%%%%
\setlength\arraycolsep{2\p@}		% TO MATCH eqnarrays<->equations
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THE EQUATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\theequation{\ifnum\c@section=0\else\thesection.\fi
			  \@arabic\c@equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURES, TABLES %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{Htbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename~\thefigure}
\newenvironment{figure}
               {\@float{figure}}
               {\end@float}
\newenvironment{figure*}
               {\@dblfloat{figure}}
               {\end@dblfloat}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}
               {\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\@dblfloat{table}}
               {\end@dblfloat}
%%-----------------------------------------------------------------%%
\newcommand{\FIGURE}[2][v]{\begin{floatingfigure}[#1]#2
                                        \end{floatingfigure}}
\newcommand{\TABLE}[2][v]{\begin{floatingtable}[#1]{#2}
                                        \end{floatingtable}}
\newcommand{\EPSFIGURE}[3][v]{\begin{floatingfigure}[#1]\epsfig{file=#2}
                                        \caption{#3}\end{floatingfigure}}
\newcommand{\TABULAR}[4][v]{\begin{floatingtable}[#1]{\begin{tabular}{#2}
					#3\end{tabular}}\caption{#4}
                                        \end{floatingtable}}
%Check below, and put automatic width ***
\newcommand{\DOUBLEFIGURE}[5][ht]{\@dblfloat{figure}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#2}}}~~~~
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#3}}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
\newcommand{\DOUBLETABLE}[5][ht]{\@dblfloat{table}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{#2}}~~~~
		\parbox{.45\textwidth}{\centerline{#3}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
%%%%%%---------------- FROM FLOATFLT PACKAGE ------------------%%%%%%%%
%% Original file `floatflt.sty', modified by F.Nesti  to:
%% be inserted in PoS.cls;
%% correct float placement when shifting past pages;
%% correct incompatibility with \marginpar;
%% correct incompatibility with \@startsection;
%% correct persisting indentation in following pars;
%% let float also at beginning of pages; 
%% avoid the widht specification.
%% 
%% Original was 1994-1996 by Mats Dahlgren <matsd@physchem.kth.se>. 
%% 
%%%%%%%%\NeedsTeXFormat{LaTeX2e}[1994/06/01]		%LEFT THIS STUFF TO 
%%%%%%%%\ProvidesPackage{floatflt}[1996/02/27 v. 1.3]	%RECONVERT TO PACKAGE.
\newcounter{OptionTest}
\if@twoside
 \setcounter{OptionTest}{0}
\else							% POS: 2side=p/1side=r
 \setcounter{OptionTest}{1}
\fi
%%%%%%%%\DeclareOption{rflt}{\setcounter{OptionTest}{1}}
%%%%%%%%\DeclareOption{lflt}{\setcounter{OptionTest}{2}} % CHOSEN.
%%%%%%%%\DeclareOption{vflt}{\setcounter{OptionTest}{0}}
%%%%%%%%\DeclareOption*{\OptionNotUsed}
%%%%%%%%\ProcessOptions
\newbox\@tmpbox
\newbox\figbox
\newbox\tabbox
\newbox\pagebox
\newcount\ffigcount
\newcount\ftabcount
\newcount\hangcount
\newcount\nosuccesstryfig
\newcount\nosuccesstrytab
\newdimen\figgutter   \figgutter=1truepc
\newdimen\tabgutter   \tabgutter=1truepc
\newdimen\fl@wd
\newdimen\fl@ht
%\newdimen\fl@gut
\newdimen\htdone      \htdone=\z@
\newdimen\pageht
\newdimen\startpageht
\newdimen\floatfltwidth
\newdimen\fltitemwidth
\newif\iftryingfig     \tryingfigfalse
\newif\iftryingtab     \tryingtabfalse
\newif\ifdoingfig      \doingfigfalse
\newif\ifdoingtab      \doingtabfalse
\newif\iffigprocessing \figprocessingfalse
\newif\iftabprocessing \tabprocessingfalse
\newif\ifpageafterfig  \pageafterfigfalse
\newif\ifpageaftertab  \pageaftertabfalse
\newif\ifoddpages
\newif\ifoutput
\newtoks\outputpretest
\def\@captype{}
%%---------------- ORRIBLE HACKS, SORRY -------------------------%%
\let\old@marginpar\marginpar				% 
\renewcommand\marginpar[1]{{\outputpretest={\outputtrue}% REDEF \marginpar.
			    \old@marginpar{#1}}}	%
\def\g@addto#1#2{{\toks@\expandafter{#1#2}%
		  \xdef#1{\the\toks@}}}%
\def\postpone@captions{%			%
%	\global\let\tmp@label\label		% REDEF \caption AND 
	\global\let\tmp@caption\caption		% \label, LATER.
	\global\let\later@capt\relax		% UN PO' PESANTI 
	\gdef\later@label{}%			% MA D'ALTRONDE...
	\let\J@ref\ref\def\ref{\protect\J@ref}% % protect ref in captions.. 
	\renewcommand\caption{\@ifnextchar[\J@@caption\J@caption}%
	\newcommand\J@caption[1]{\gdef\later@capt{\tmp@caption{##1}}}% LOCAL!!
	\newcommand\J@@caption[2][v]%
				{\gdef\later@capt{\tmp@caption[##1]{##2}}}% LOCAL!!
	\renewcommand\@@label[1]{\egroup\name{ref-##1}%	% TAG WHERE CALLED, AT LEAST,
			       \if@draft\norm@note{}{LAB: ##1}\fi% & DRAFTNOTE.
			       \g@addto\later@label{\old@label{##1}}}%
			}
\AtEndDocument{\iftryingfig\PoS@warnl{Floating figure \the\ffigcount\space
					remains undone}\fi
		\iftryingtab\PoS@warnl{Floating table \the\ftabcount\space
					remains undone}\fi}
%%----------------- FIGURE ---------------------------------------%%
\newenvironment{floatingfigure}[1][v]%
{\@tfor \@tempa :=#1\do {\xdef\@fside{\@tempa}}%
 \global\advance\ffigcount by 1%
 \iffigprocessing {\count0=\ffigcount\advance\count0 by -1%
   		   \PoS@warnl{Floating figures \the\count0\space\space and
       			\the\ffigcount\space colliding}}\fi
 \iftabprocessing  \PoS@warnl{Floating table \the\ftabcount\space and 
			floating figure \the\ffigcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of figbox %HBOX FOR AUTO WIDTH!
}
{%
\egroup%				% CALCULATE WIDTH (NO CAPTION FOR NOW)
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
 \global\setbox\figbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{figure}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
 \global\figprocessingtrue
 \global\everypar={\tryfig\oldeverypar}% must be set globally!
 \figinsert\par
\else%					% ELSE NORMAL LATEX FIGURE, SIGH.
 \if\@fside v \def\@fside{ht}\fi
 \ifdim\floatfltwidth<\columnwidth
    \def\@@tempa{\@float{figure}[}\let\@@tempb\end@float
 \else
    \def\@@tempa{\@dblfloat{figure}[}\let\@@tempb\end@dblfloat
 \fi
 \expandafter\@@tempa\@fside]\center\unhbox\@tmpbox\later@capt\later@label\@@tempb
\fi
}
%%------------ TABLE ----------------------------------------------%%
\newenvironment{floatingtable}[1][v]%
{\@tfor \@tempa :=#1\do {\global\edef\@tside{\@tempa}}%
 \global\advance\ftabcount by 1%
 \iftabprocessing {\count0=\ftabcount\advance\count0 by -1%
     		   \PoS@warnl{Floating tables \the\count0\space
            		\space and \the\ftabcount \space colliding}}\fi
 \iffigprocessing  \PoS@warnl{Floating figure \the\ffigcount\space and 
			floating table \the\ftabcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of tabbox, ACTUALLY AN HBOX.
}
{%
\egroup% end of \tabbox, 		% ACTUALLY \@tmpbox
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
  \global\setbox\tabbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{table}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
  \global\tabprocessingtrue
  \global\everypar={\trytab\oldeverypar}%
  \tabinsert\par%
\else%					% ELSE NORMAL LATEX TABLE.
%  \PoS@mess{Floating table \the\ftabcount\space is 
%			wide becomes a LaTeX float}%
  \ifdim\floatfltwidth<1.1\columnwidth
    \if\@tside v \def\@tside{ht}\fi
    \def\@@tempa{\@float{table}[}\let\@@tempb\end@float
  \else
    \if\@tside v \def\@tside{t}\fi
    \def\@@tempa{\@dblfloat{table}[}\let\@@tempb\end@dblfloat
  \fi
  \expandafter\@@tempa\@tside]%		% ACTUALLY CALL THE LATEX FLOAT
  \center\unhbox\@tmpbox\later@capt\later@label
  \@@tempb
\fi%
}
%----------- prepare for tries ----------------------------%
\def\figinsert{%
   \global\nosuccesstryfig=0%
   \global\outputpretest={\do@test}%
   \global\tryingfigtrue \global\doingfigfalse%
   \global\pageafterfigfalse}%
\def\tabinsert{%
   \global\nosuccesstrytab=0%
   \global\outputpretest={\do@test}%
   \global\tryingtabtrue \global\doingtabfalse%
   \global\pageaftertabfalse}%
%----------- init -----------------------------------------%
\AtBeginDocument{%
 \edef\oldoutput{\the\output}
 \output={\the\outputpretest\ifoutput\oldoutput\fi}%
 \outputpretest={\outputtrue}%
 \edef\oldeverypar{\the\everypar}% PERCHE' NESSUNO LO RIMETTE PIU' A POSTO?***
}
%---- tests during \outputpretest -------------------------%
\def\do@test{%
   \ifnum\outputpenalty=-10005
%	\output
     \setbox\pagebox=\vbox{\unvbox255}%
     \global\pageht=\ht\pagebox
     \global\outputfalse
     \unvbox\pagebox
     \dimen0=\pageht\advance\dimen0 by 2 \baselineskip
     \ifdim\dimen0>\vsize\global\pageht\z@\fi
   \else
     \global\outputtrue
     \ifnum\outputpenalty>-\@Mi			%ie \marginpar's give penalty.
	\ifdoingtab\global\pageaftertabtrue\fi
	\ifdoingfig\global\pageafterfigtrue\fi
     \fi
   \fi}%
%-------- check for side ----------------------------------%
\def\chk@side#1{% DEFINED \fl@sid, BUT IF CHOSEN A DEFAULT, ELIMINATE ALL ***
	{\edef\fl@sid{#1}%
	  \if\fl@sid r\global\oddpagestrue\fi
          \if\fl@sid l\global\oddpagesfalse\fi
          \if\fl@sid p%
              \ifodd\c@page\global\oddpagesfalse
                \else\global\oddpagestrue\fi
          \fi
          \if\fl@sid v%
             \ifnum\theOptionTest=0%
                 \ifodd\c@page\global\oddpagesfalse
                   \else\global\oddpagestrue\fi
             \else
                  \ifodd\theOptionTest\global\oddpagestrue
                    \else\global\oddpagesfalse\fi
             \fi
          \fi
         }}%
%-------- get point in page -------------------------------%
\def\get@pageht{{\everypar={\relax}\setbox0=\lastbox
       		\parindent=\wd0 \parskip=\z@ \par
         	\penalty-10005 \leavevmode}}%
%-------- try at everypar ---------------------------------%
\def\tryfig{%
	\global\fl@ht\ht\figbox
	\global\fl@wd\wd\figbox
	\global\let\fl@gut\figgutter
      \iftryingfig
	\get@pageht
	\dimen0=\vsize
	\advance\dimen0 by -\pageht
	\advance\dimen0 by -2\baselineskip
	\ifdim\dimen0>\fl@ht
	  \chk@side\@fside
	  \dimen0=0.3\baselineskip
	  \vrule depth \dimen0 width \z@%height 1.5\baselineskip
	  \vadjust{\kern -\dimen0
	  \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\figbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\figbox\hss}%
             \fi
             \vss}\null}}%
	  \global\tryingfigfalse
	  \global\doingfigtrue
	  \global\startpageht=\pageht
	  \global\htdone=\z@
	  \dohang
	  \ifnum\nosuccesstryfig>0%
	   \PoS@mess{Flt. fig. \the\ffigcount\space set on page \the\count0, 
	 		shifted \the\nosuccesstryfig\space par(s) forward}%
%	  \else
%	   \PoS@mess{Floating figure \the\ffigcount\space 
%			set on page \the\count0}%
	  \fi
	\else
          \global\advance\nosuccesstryfig by 1
	\fi
      \else%				% IF NOT TRYING
	\ifdoingfig
	  \get@pageht
	  \global\htdone=\pageht
	  \global\advance\htdone by -\startpageht
	  \ifpageafterfig
	    \global\doingfigfalse% IN CASE A PAGEBREAK JUST BELOW?
	  \else
	    \dimen0=\fl@ht
	    \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
%	    \typeout{FLOAT HT: \the\dimen0, HTDONE: \the\htdone}
	    \ifdim\htdone<\dimen0%
		\dohang
	    \else
		\global\doingfigfalse
	    \fi
	  \fi
	  \ifdoingfig\else\global\figprocessingfalse\fi% IF NO MORE DOING.
	\else
	  \global\outputpretest={\outputtrue}% NOT RESTORE EVPAR IF NOT DOING?
	\fi%			% END IF DOING
      \fi%			% END IF TRYING
}
\def\trytab{%
	\global\fl@ht\ht\tabbox
	\global\fl@wd\wd\tabbox
	\global\let\fl@gut\tabgutter
       \iftryingtab
	\get@pageht
       \dimen0=\vsize
       \advance\dimen0 by -\pageht
       \advance\dimen0 by -2\baselineskip
       \ifdim\dimen0>\fl@ht
	 \chk@side\@tside
         \dimen0=0.3\baselineskip
         \vrule depth \dimen0 width \z@
         \vadjust{\kern -\dimen0
         \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\tabbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\tabbox\hss}%
             \fi
             \vss}\null}}%
       \global\tryingtabfalse
       \global\doingtabtrue
       \global\startpageht=\pageht
       \global\htdone=\z@
       \dohang
       \ifnum\nosuccesstrytab>0%
	\PoS@mess{Flt. tab. \the\ftabcount\space set on page \the\count0, 
			shifted \the\nosuccesstrytab\space par(s) forward}%
       \fi
     \else
       \global\advance\nosuccesstrytab by 1
     \fi
     \else
     \ifdoingtab
       \get@pageht
    \global\htdone=\pageht
    \global\advance\htdone by -\startpageht
    \ifpageaftertab
      \global\doingtabfalse
    \else
      \dimen0=\fl@ht
      \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
      \ifdim\htdone<\dimen0%
         \dohang
      \else
         \global\doingtabfalse
      \fi
    \fi
    \ifdoingtab\relax\else\global\tabprocessingfalse\fi
  \else
    \global\outputpretest={\outputtrue}%
  \fi
\fi
}
%----- hanging lord -----------------------------%
\def\dohang{%
   \dimen0=\fl@ht
   \advance\dimen0 by -\htdone
   \advance\dimen0 by 1.999\baselineskip	% (16/12/98) WAS 1.49 BUT
   \hangcount=\dimen0				% TEX ROUNDS ON STRICT INTEGERS
   \divide\hangcount by \baselineskip		% IN THIS DIVISION!
     \dimen0=\fl@wd
     \advance\dimen0 by \fl@gut
     \ifoddpages
       \global\hangindent=-\dimen0% placing right
     \else 
       \global\hangindent=\dimen0% placing left
     \fi
   \global\hangafter=-\hangcount
%   \fi
}
%----------------------- TWO NEWITEMS ---------------------%
\newcommand{\fltitem}[2][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item \parbox[t]{\fltitemwidth}{#2}\\[#1]}
\newcommand{\fltditem}[3][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item[#2] \parbox[t]{\fltitemwidth}{#3}\\[#1]}
%%%%%%\endinput
%% 
%% End of ex-file `floatflt.sty'.

%%% this is a modification to the standard latex to make bottom
%%% figures appear above the footnote
% problema: se nella stessa pagina ci sono una figura piccola e una
% [b] o [t] dopo di essa quella piccola viene a sinistra
% ma questo succede anche senza questa patch!
% e con o senza footnote.

\newbox\JCAP@outputbox
\gdef \@makecol {%
   \ifvoid\footins
     \setbox\@outputbox \box\@cclv
   \else
     \setbox\@outputbox \vbox {%
       \boxmaxdepth \@maxdepth
       \@tempdima\dp\@cclv
	\unvbox \@outputbox
       \unvbox \@cclv
       \vskip-\@tempdima
     }%
     \setbox\JCAP@outputbox \vbox {%
       \vskip \skip\footins
       \color@begingroup
         \normalcolor
         \footnoterule
         \unvbox \footins
       \color@endgroup
       }%
   \fi
   \xdef\@freelist{\@freelist\@midlist}%
   \global \let \@midlist \@empty
   \@combinefloats
   \ifvbox\@kludgeins
     \@makespecialcolbox
   \else
     \setbox\@outputbox \vbox to\@colht {%
       \@texttop
       \dimen@ \dp\@outputbox
       \unvbox \@outputbox
       \vskip -\dimen@
       \unvbox\JCAP@outputbox
       \@textbottom
       }%
   \fi
   \global \maxdepth \@maxdepth
}
%%% end of the patch

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{8\p@ plus 1pt minus 2pt}
\setlength\belowcaptionskip{0\p@}
\long\def\@makecaption#1#2{%
  \if@hyper{\edef\@pippo{the\@captype}
	    \name{\@captype\expandafter\csname\@pippo\endcsname}}\fi%
  \vskip\abovecaptionskip
 {\let\label\@gobble%				% FN 10.2.97 REMOVED LATEX BUG:
  \let\index\@gobble%				% LARGE CAPTIONS PROCESS LABEL
  \let\glossary\@gobble%			% TWO TIMES.
  \sbox\@tempboxa{\small {\bfseries #1:} #2}%	% 
  \global\dimen0\wd\@tempboxa}%			%
  \ifdim \dimen0 >\hsize
    \small {\bfseries #1:} #2\par
  \else
    \global\@minipagefalse \sbox\@tempboxa{\small {\bfseries #1:} #2}%
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FONTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TOC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\tocsecs{}
\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
\if@todotoc
    \section*{\contentsname\label{-TOC-}}
    \@starttoc{toc}%
    \gdef\tableofcontents{\PoS@igno{\tableofcontents\space already done}}
\else
\PoS@ignol{\tableofcontents. Use option [toc]}
\fi}
\newcommand*\l@part[2]{\def\hyp@typ{part}%	
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries \tocsecs#1\hfil \hb@xt@\@pnumwidth{\hss
		\intPlink{\hash pag#2}{#2}}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{\def\hyp@typ{sec}%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.8em}%	%WIDTH OF SECT. N.
    \begingroup
      \let\d@t.%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
        \tocsecs#1\nobreak\hfil %HREF HERE WOULD GET ALSO THE TITLE(...)
        \nobreak\hb@xt@\@pnumwidth{\hss \intPlink{\hash pag#2}{#2}}\par
    \endgroup
  \fi}

\newcommand*\l@subsection{\def\hyp@typ{sec}\@tocline{2}{1.8em}{2.3em}}
\newcommand*\l@subsubsection{\def\hyp@typ{sec}\@tocline{3}{4.1em}{3.1em}}
\newcommand*\l@paragraph{\def\hyp@typ{sec}\@tocline{4}{7.2em}{4.3em}}
\newcommand*\l@subparagraph{\def\hyp@typ{sec}\@tocline{5}{10.5em}{5em}}

\if@hyper
  \let\old@dtl\@dottedtocline
  \def\@dottedtocline#1#2#3#4#5{\old@dtl{#1}{#2}{#3}{#4}{%
						\intPlink{\hash pag#5}{#5}}}
\fi

\def\@tocline#1#2#3#4#5{%
  \ifnum #1>\c@tocdepth \else
    \vskip \z@ \@plus.2\p@
    {\leftskip #2\relax \rightskip \@tocrmarg \parfillskip -\rightskip
     \parindent #2\relax\@afterindenttrue
     \interlinepenalty\@M
     \leavevmode
     \@tempdima #3\relax
     \advance\leftskip \@tempdima \null\nobreak\hskip -\leftskip
     {#4}\nobreak
     \hfill
     \nobreak
     \hb@xt@\@pnumwidth{\hfil\normalfont \normalcolor \intPlink{\hash pag#5}{#5}}%
     \par}%
  \fi}


%%%%%%%%%%%%%%%%%%%%%% LIST OF FIGURES AND TABLES %%%%%%%%%%%%%%%%%%%%%
\if@draft			% ONLY IF DRAFT! ... 
 \newcommand\listoffigures{%
     \section*{\listfigurename
       \@mkboth{\MakeUppercase\listfigurename}%
               {\MakeUppercase\listfigurename}}%
     \@starttoc{lof}%
     }
 \newcommand*\l@figure{\def\hyp@typ{figure}\@dottedtocline{1}{1.5em}{2.3em}}
 \newcommand\listoftables{%
     \section*{\listtablename
       \@mkboth{%
           \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
     \@starttoc{lot}%
     }
 \newcommand*\l@table{\def\hyp@typ{table}\@dottedtocline{1}{1.5em}{2.3em}}
\else
 \newcommand\listoffigures{\PoS@ignol{List of figures (draft mode only)}}
 \newcommand\listoftables{\PoS@ignol{List of tables (draft mode only)}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BIBLIOGRAPHY %%%%%%%%%%%%%%%%%%%%%%%%%%%%***
\newdimen\bibindent
\setlength\bibindent{1.5em}
\newenvironment{thebibliography}[1]%	%UNFORTUNATELY MODIFIED..
     {\bgroup\raggedright\small\section*{\refname
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}}%
      \list{\name{bib\@arabic\c@enumiv}% HOPE!
	    \@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist\egroup}
\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\if@draft
 \let\old@bbt\@bibitem\let\old@lbbt\@lbibitem% LOOK THE DISASTER HERE BELOW.
 \def\@lbibitem[#1]#2{\old@lbbt[#1]{#2}\reversemarginpar{\sf\bfseries\small#2}}
 \def\@bibitem#1{\old@bbt{#1}\reversemarginpar{\sf\bfseries\small#1}}
\fi
\let\@openbib@code\@empty
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BopHook %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand\PoS[1]{\PoSsplit@ident#1.\@PoStrue%
\def\bop{%
\rotatebox{-90}{%
    \makebox[0cm][r]{%
      \raisebox{1.0892\textwidth}[0pt][0pt]{%
      \fontsize{30}{12}\selectfont\tt 
      \textcolor[rgb]{0.8,0.8,0.8}{#1}\hspace{241.23pt}}}}}
\let\PoS\gobble}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\skip\footins = 1\bigskipamount plus 2pt minus 4pt

\addtolength{\footnotesep}{1pt}
\renewcommand\footnoterule{%	% NO HYPER...
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}
\newcommand\@makefntext[1]{%
    \parindent 20.39995pt%
%\setlength\parindent{20pt} 
   \noindent
    \hb@xt@\parindent{\hss\@makefnmark}#1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\contentsname{Contents}
\if@draft\newcommand\listfigurename{List of figures}
	 \newcommand\listtablename{List of tables}\fi
\newcommand\refname{References}
\newcommand\indexname{Index}
\newcommand\figurename{Figure}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{Abstract:}
\newcommand\acknowlname{Acknowledgments}

\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}

\setlength\columnsep{20\p@}
\setlength\columnseprule{0\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEFAULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagestyle{PoS}
\pagenumbering{arabic}
\@addtoreset{equation}{section}
		\let\pagestyle\@gobble
		\let\thispagestyle\@gobble
		\let\pagenumbering\@gobble
\onecolumn
						
% FOR REQUESTED FRONTMATTER ...
\AtBeginDocument{\bgroup%		SOME NICE (LOCAL) MESSAGES... 
	\def\@APPwarn#1{\PoS@warnl{\protect#1 should appear 
					before \protect\begin{document}}}%
	\def\@APPerr#1{\ClassError{PoS}{\protect#1 should appear 
					before \protect\begin{document}}}%
	\if@author\else\@APPerr{Some \protect\author{...}}\fi
	\if@abstract\else\@APPerr{\abstract{...}}\fi
	\if@conf\else\@APPerr{\FullConference{...}}\fi
	\if@shorttitle\else\@APPerr{\ShortTitle{...}}\fi
	\if@PoS\else\@APPerr{\PoS{PoS(CONF)nnn}}\fi
	\egroup
	\auto@maketitle
	\if@speaker\else\PoS@warnl{One \protect\speaker{...}
			must be specified among authors}\fi
			\if@dblspeak\PoS@warnl{A single \protect\speaker{...}
			should appear in proceedings}\fi
}
\endinput
%% 
%% End of file `PoS3.cls'.

